Friable averages of oscillating multiplicative functions

We evaluate friable averages of arithmetic functions whose Dirichlet series is analytically close to some negative power of the Riemann zeta function. We obtain asymptotic expansions resembling those provided by the Selberg-Delange method in the non-friable case. An application is given to summing truncated versions of such functions.

==> itenn.tex <==
  % MISE EN PAGE 
  
 \def\oui{oui} 
  
  %\magnification 1100
\ifx\arXiv\oui
\else
 \pdfpagewidth=210truemm
 \pdfpageheight=297truemm 
\fi
  
  %
  % Definitions pour les notes en bas de page
  % [Format : \note{texte de la note} avec numerotation automatique]
  %
  

  %
  %\anote=\footnote de plain (2 arguments)
  %
  \let\footnotea=\footnote
  \def\anote#1#2{\footnotea{\hbox{$^{#1}$}}{\eightpoint#2}}  
  \catcode`@=12 % at signs are no longer letters

  %reference de note
 \def\defrefnote#1{\definexref{#1}{{\the\footnotenumber}}{refnotes}}
 \def\refnote#1{\ref{#1}}
  
  %
  % Fin notes
  %
  
  
  %\def\eqlgno#1{$$\leqalignno{#1}$$}

\ifx\couleurs\oui
\input graphicx
 \pdfpagewidth=210truemm
 \pdfpageheight=297truemm 
 \voffset=-5mm
\fi

\input eplain.tex
\expandafter\def\expandafter\newdimen\expandafter{\newdimen}



% couleurs
% Attention : \illust et graphicx nŽcessitent \couleurs={oui}
\ifx\couleurs\oui
%\expandafter\def\expandafter\newdimen\expandafter{\newdimen}
\beginpackages
\usepackage{color}
\endpackages 
 \pdfpagewidth=210truemm
 \pdfpageheight=297truemm 
\long\def\rge#1{{\color{red}#1}}
\long\def\bl#1{{\color{blue}#1}}
\long\def\vrt#1{{\color[cmyk]{0.9, .1, 0.8, 0.2}#1}}
\long\def\bleuGT{\special{color cmyk 1. .25 0.0 0.0}}
\definecolor{bleu-iecn}{cmyk}{.98,.13,.1,.55}
\long\def\BleuIECN#1{{\color{bleu-iecn}#1}}
\long\def\vlt#1{{\color[cmyk]{.3, 1, .2, 0}#1}}
\long\def\org#1{{\color[cmyk]{.0, .75, 1, .15}#1}}
\else
\long\def\rge#1{#1}
\long\def\bl#1{#1}
\long\def\vrt#1{#1}
\long\def\BleuIECN#1{#1}
\long\def\vlt#1{#1}
\long\def\org#1{#1}
\fi


\makeatletter
\def\numberedfootnote{%
ÊÊ\global\advance\footnotenumber by 1
ÊÊ\@eplainfootnote{{\number\footnotenumber}}%
}%
\def\makecolumns#1/#2 {\par \begingroup
ÊÊ \@columndepth = #1
ÊÊ \advance\@columndepth by -1
ÊÊ \divide \@columndepth by #2
ÊÊ \advance\@columndepth by 1
ÊÊ \@linestogoincolumn = \@columndepth
ÊÊ \@linestogo = #1
ÊÊ \currentcolumn = 1
ÊÊ \def\@endcolumnactions{%
ÊÊÊÊÊÊ\ifnum \@linestogo<2
ÊÊÊÊÊÊÊÊ \the\crtok \egroup \endgroup \par % End \valign and \makecolumns.
ÊÊÊÊÊÊ\else
ÊÊÊÊÊÊÊÊ \global\advance\@linestogo by -1
ÊÊÊÊÊÊÊÊ \ifnum\@linestogoincolumn<2
ÊÊÊÊÊÊÊÊÊÊÊÊ\global\advance\currentcolumn by 1
ÊÊÊÊÊÊÊÊÊÊÊÊ\global\@linestogoincolumn = \@columndepth
ÊÊÊÊÊÊÊÊÊÊÊÊ\the\crtok
ÊÊÊÊÊÊÊÊ \else
ÊÊÊÊÊÊÊÊÊÊÊÊ&\global\advance\@linestogoincolumn by -1
ÊÊÊÊÊÊÊÊ \fi
ÊÊÊÊÊÊ\fi
ÊÊ }%
ÊÊ \makeactive\^^M
ÊÊ \letreturn \@endcolumnactions
ÊÊ \@columnwidth = \hsize
ÊÊÊÊ \advance\@columnwidth by -\parindent
ÊÊÊÊ \divide\@columnwidth by #2
ÊÊ \penalty\abovecolumnspenalty
ÊÊ \noindent % It's not a paragraph (usually).
ÊÊ \valign\bgroup
ÊÊÊÊ &\hbox to \@columnwidth{\strut \hsize = \@columnwidth ##\hfil}\cr
}%
\makeatother

\lefteqnumbers
% choix numerotation gauche ou droite: defaut=gauche, \numadroite{oui} -> a droite
   \def\testd{oui}
   \def\choixlat{\ifx\numadroite\testd\righteqnumbers
            \else  \lefteqnumbers\fi}
    \choixlat

% modif format note
\catcode`@=\letter
\def\@eplainfootnote#1{\let\@sf\empty % parameter #2 (the text) is read later
  \ifhmode\edef\@sf{\spacefactor\the\spacefactor}\/\fi
  \global\advance\hlfootlabelnumber by 1
  \hlstart@impl{foot}{\hlfootlabel}%
  \hldest@impl{footback}{\hlfootbacklabel}%
  \hbox{$^{(#1)}$}%
  \hlend@impl{foot}%
  \@sf\vfootnote{#1.}%
}%
\catcode`@=\other

  \interfootnoteskip=0pt
  \let\note=\numberedfootnote
  \everyfootnote={\eightpoint\leftskip=5truemm\rightskip5truemm}
  
  \hsize150truemm\vsize 240truemm\hoffset=5truemm
  
  \def\dimstand{\hsize 150truemm\vsize 250truemm\hoffset=8truemm\voffset=5truemm}
  \def\dimart{\hsize126truemm\vsize186truemm\hoffset16truemm\voffset=24truemm}
  \pretolerance=500\tolerance=1000\brokenpenalty=5000
  \parindent3mm
  
  \countdef\temps=170
  \temps=\time
  \countdef\nminutes=171{\nminutes = \time}
  \countdef\nheure=172
  \def\heure{\begingroup                     % heure a la francaise
     \temps = \time \divide\temps by 60
     \nheure = \temps                        % l'heure, de 0 \`a 23
     \nminutes = \time
     \multiply\temps by 60
     \advance\nminutes by -\temps            % Les minutes, de 0 a 59.
     \ifnum\nminutes<10 \toks1 = {0}%
     \else\toks1 = {}%
     \fi
     \number\nheure h\the\toks1 \number\nminutes  
  \endgroup}%
  
  
  \newcount\chstart
  \chstart=\pageno
 \headline={\ifnum\pageno=\chstart {\hfill} \else {\hss \tenrm --\ \folio\ --\hss}\fi}
  \footline={\hfill}
  \normalbaselines
  \frenchspacing
    \def\dater{\vglue-10mm\rightline{(\the\day/\the\month/\the\year)}}
  \def\dateheure{\vglue-10mm\rightline{(\the\day/\the\month/\the\year,\ \heure)}}
\def\raggedleft{\leftskip=0pt plus 2em\parfillskip=0pt
\spaceskip=.3333em\xspaceskip=.5em} % justification ˆ droite

  
  \newif\ifpagetitre \pagetitretrue
\newtoks\hautpagetitre \hautpagetitre={\hfill}
\newtoks\baspagetitre \baspagetitre={\hfill}
\newtoks\auteurcourant \auteurcourant={\hfill}
\newtoks\titrecourant \titrecourant={\hfill}
\newtoks\hautpagegauche
\newtoks\hautpagedroite
\newtoks\hautpagemilieu
\hautpagemilieu={\tenrm\hfil -- \folio\ -- \hfil}
\hautpagegauche={\ifx\midfolio\oui\the\hautpagemilieu\else\tenrm\folio\hfill\the\auteurcourant\hfill\fi}
\hautpagedroite={\ifx\midfolio\oui\the\hautpagemilieu\else\hfill\the\titrecourant\hfill\tenrm\folio\fi}
\newtoks\baspagegauche \baspagegauche={\hfil}
\newtoks\baspagedroite \baspagedroite={\hfil}
\headline={\ifpagetitre\the\hautpagetitre
\else\ifodd\pageno\the\hautpagedroite\else\the\hautpagegauche\fi\fi }
\footline={\ifpagetitre\the\baspagetitre
\else\ifodd\pageno\the\baspagedroite
\else\the\baspagegauche\fi\fi \global\pagetitrefalse}

\def\nopagenumber{\headline={\hfill}\footline={\hfill}}
%\def\numpgsuiv{ \chstart=\pageno\pageno=\chstart}

\def\pageblanche{\vfill\eject\pagetitretrue
\null\vfill\eject
\pagetitretrue
}
\def\chgtpage{\ifodd\pageno \else
\pageblanche \fi \pagetitretrue\titreun=0\footnotenumber=0}

\def\chgtpageincrtitreun{\ifodd\pageno \else
\pageblanche \fi \pagetitretrue\footnotenumber=0}

\def\majnombres{\ifodd\pageno \else
\pageblanche \fi \pagetitretrue\hautpoly\titreun=0\footnotenumber=0}
\def\raznombres{\titreun=0 \footnotenumber=0 \eqnumber=0}

\def\hautspages#1#2{\auteurcourant={\ninepcap#1}\titrecourant={\nineit#2}}

\ifnum\chstart=\pageno \pagetitretrue\fi
%\ifnum\pageno=\chstartÊ\pagetitretrue \fi
  
  %pour eviter les rectangles noirs:
  %\overfullrule=Opt
  % pour que les @ soient des lettres
  \def\signeat{\catcode`@=11}
  
  
  %% pour aller a la ligne dans un \proclaim:
  \def\PAR{\par}
  
  %% Note en marge gauche
  \def\leftnote#1{\vadjust{\setbox1=\vtop{\hsize 20mm\parindent=0pt\eightpoint
  \baselineskip=9pt\rightskip=4mm plus 4mm\vskip-4.7mm#1}\hbox{\kern-2cm\smash{\box1}}}}
  \def\OK{\leftnote{\bf OK ?}}

  %% Pour couper automatiquement un titre trop long
  
  \def\raggedcenter{\leftskip=20pt plus 10em  % reglages initial 4em
       \rightskip=\leftskip 
        \parfillskip=0pt 
         \spaceskip=.3333em \xspaceskip=.5em 
          \pretolerance=9999 \tolerance=9999
           \hyphenpenalty=9999 \exhyphenpenalty=9999 }
           
  \def\titrecentre#1{{\parindent0mm\raggedcenter
       \spaceskip=.6em plus .2em minus .2em\xspaceskip=.6em plus .2em minus .2em
        \tit#1\par}}
        
% entourer un texte par un filet

\def\boxit#1#2{\vbox{\hrule\hbox{\vrule\vbox spread#1{\vfil\hbox spread#1{\hfil#2\hfil}\vfil}%
\vrule}\hrule}}
\def\entourer#1#2{\setbox1=\vtop{#2}\boxit{#1}{\box1}}


  
  %%%%%% D\'ebut num\'erotation automatique des paragraphes et/ou des enonces

  
  \def\oui{oui}
  
\def\fontetitreun{\ifx\paradouze\oui\douzepts\gpdouze\twelvebf\textfont1=\twelveib\else
\quatorzepts\gpquatorze\fourteenbf\fi}

\def\fontetitreunl{\douzepts\textfont1=\twelveib\scriptfont1=\tenib\fourteenti}
 
 \def\fontetitredeux{\textfont1=\eleveni\ifx\paradouze\oui\onzepts\scriptfont1=\ninei\elevenit\else
                        \douzepts\twelveit\fi}
 
   \def\fontetitredeuxb{\ifx\paradouze\oui\onzepts\eleventi\gponze\textfont1=\elevenib\scriptfont1=\nineib
                         \else\douzepts\twelveti\scriptfont1=\twelveib\scriptfont1=\tenib\gpdouze\fi}
                         
\def\fontetitredeuxl{\onzepts\textfont1=\elevenbf\scriptfont1=\ninebf\twelvebf}
  
\def\fontetitretrois{\textfont0=\elevenrm\scriptfont0=\eightrm\textfont1=\eleveni
                      \scriptfont1=\eighti\scriptscriptfont1=\sixi\elevenit}
                      
\def\fontetitrequatre{\textfont0=\elevenrm\scriptfont0=\eightrm\textfont1=\eleveni
                      \scriptfont1=\eighti\scriptscriptfont1=\sixi\elevenrm}
  
  \newcount\titreun\titreun=0
  \newcount\titredeux\titredeux=0
  \newcount\titretrois\titretrois=0
  \newcount\titrequatre\titrequatre=0
  \newcount\enonce\enonce=0
  
  \def\incr#1{\global\advance#1 by 1 {\the #1}}
  \def\avance#1{\global\advance#1 by 1}
  \def\init#1{\global#1=0}
  
  \long\def\Indentation#1#2{\setbox10=\hbox{\fontetitreun#1}
  	                    \ifdim\wd10 < 4mm
                         \setbox10=\hbox to 4mm{\box10\hfill}
                       \else\ifdim\wd10 < 6mm
                         \setbox10=\hbox to 6mm{\box10\hfill}
  	                    \else\ifdim\wd10 < 8mm
                         \setbox10=\hbox to 8mm{\box10\hfill}
                       \else\ifdim\wd10 < 12mm
                         \setbox10=\hbox to 12mm{\box10\hfill}
                       \fi\fi\fi\fi
                       \dimen10=\hsize
                       \advance \dimen10 by -\wd10
                       \noindent \box10 %
                       \ignorespaces
                       \hbox{\vtop{\hsize=\dimen10\raggedright\noindent\fontetitreun#2}}}
  
 
  \long\def\paraun#1{\removelastskip\par\medskip\goodbreak\vskip0pt plus.01\vsize\penalty-100
                \vskip0pt plus-.01\vsize
  	              \init{\titredeux}\ifnum\optionparag=1{\init\eqnumber\init\enonce}\else{}\fi
                  \goodbreak{\fontetitreun
  	                \Indentation{\incr{\titreun}.\ }{\fontetitreun #1\par}}\nobreak\medskip}

                   
 %
 % titres de paragraphes centres
 %
 \long\def\paraunc#1{\removelastskip\par\bigskip\goodbreak\vskip0pt plus.01\vsize\penalty-100
                \vskip0pt plus-.01\vsize
  	              \init{\titredeux}
                 \ifnum\optionparag=1{\init{\eqnumber}\init\enonce}\else{}\fi
                  \goodbreak
  	                {\parindent0mm\raggedcenter\fontetitreun\incr{\titreun}.\ 
                     \fontetitreun #1\par}\nobreak\medskip}
                     
% paragraphes de niveau 1 numŽrotŽs avec des chiffres romains
\newtoks\titreunl
\titreunl={\ifnum\titreun=1{I}\fi%
\ifnum\titreun=2{II}\fi%
\ifnum\titreun=3{III}\fi%
\ifnum\titreun=4{IV}\fi%
\ifnum\titreun=5{V}\fi%
\ifnum\titreun=6{VI}\fi%
\ifnum\titreun=7{VII}\fi%
\ifnum\titreun=8{VIII}\fi%
\ifnum\titreun=9{IX}\fi%
\ifnum\titreun=10{X}\fi%
\ifnum\titreun=11{XI}\fi%
\ifnum\titreun=12{XII}\fi%
\ifnum\titreun=13{XIII}\fi%
}
\long\def\paraunl#1{\removelastskip\par\bigskip\bigskip\goodbreak\vskip0pt plus.01\vsize\penalty-100
                \vskip0pt plus-.01\vsize
  	              \init{\titredeux}\ifnum\optionparag=1{\init\eqnumber\init\enonce}\else{}\fi
                  \goodbreak{\fontetitreunl
  	                \Indentation{\global\advance\titreun by 1{\the\titreunl}.\ }{\fontetitreunl #1\par}}\nobreak\smallskip}


% paragraphes de niveaux 2
  
  \long\def\paradeux#1{\init{\titretrois}\vskip0pt plus.01\vsize\penalty-10
                \vskip0pt plus-.01\vsize\ifx \elie\oui\medskip\ifnum\titredeux>0\medskip\fi\fi
                 \Indentation{\fontetitredeux\the\titreun${\cdot}$\incr{\titredeux}.}
                              {\fontetitredeux\textfont1=\eleveni#1}\nobreak\par }
  
  \long\def\paradeuxb#1{\init{\titretrois}\vskip0pt plus.001\vsize\penalty-10
                \vskip0pt plus-.01\vsize{\ifx \elie\oui\medskip\ifnum\titredeux>0\medskip\fi\fi
                  \Indentation
  {\fontetitredeuxb\the\titreun${\cdot}$\incr{\titredeux}.}{ \fontetitredeuxb#1}}\nobreak
\smallskip}

% paragraphes de niveau 2 numŽrotŽs avec des lettres capitales 
\newtoks\titredeuxl
\titredeuxl={\ifnum\titredeux=1{A}\fi%
\ifnum\titredeux=2{B}\fi%
\ifnum\titredeux=3{C}\fi%
\ifnum\titredeux=4{D}\fi%
\ifnum\titredeux=5{E}\fi%
\ifnum\titredeux=6{F}\fi%
\ifnum\titredeux=7{G}\fi%
\ifnum\titredeux=8{H}\fi%
\ifnum\titredeux=9{I}\fi%
\ifnum\titredeux=10{J}\fi%
\ifnum\titredeux=11{K}\fi%
\ifnum\titredeux=12{L}\fi%
\ifnum\titredeux=13{M}\fi%
}
 \long\def\paradeuxl#1{\init{\titretrois}\vskip0pt plus.001\vsize\penalty-10
                \vskip0pt plus-.01
                \vsize \bigskip%
                  \Indentation
     {\fontetitredeuxl\global\advance\titredeux by 1
  \quad \the\titreunl${\cdot}$\the\titredeuxl.}{ \fontetitredeuxl#1}
  \removelastskip\nobreak\smallskip}
  
% paragraphes de niveaux 3

  \long\def\paratrois#1{\init{\titrequatre}\ifdim\lastskip<\smallskipamount
                \removelastskip\smallskip\fi
                 \vskip0pt plus.01\vsize\penalty-10
                  \vskip0pt
plus-.01\vsize{\ifx \elie\oui\ifnum\titretrois>0\medskip\fi\fi
\Indentation{\fontetitretrois\the\titreun${\cdot}$\the\titredeux${\cdot}$\incr{\titretrois}.\ }
  {\hskip0mm\baselineskip=14pt\fontetitretrois#1}\nobreak\smallskip}}
  
 % paragraphes de niveau 3 numŽrotŽs avec des chiffres mais niveaux 1 et 2 chiffres romains et lettres 
  
  \long\def\paratroisl#1{\init{\titrequatre}\ifdim\lastskip<\smallskipamount
                \removelastskip\fi
                 \vskip0pt plus.01\vsize\penalty-10
                  \vskip0pt
plus-.01\vsize\ifx \elie\oui\bigskip
\fi
\Indentation{\fontetitretrois\quad \quad \the\titreunl{${\cdot}$}\the\titredeuxl${\cdot}$\incr{\titretrois}.\ }
  {\hskip0mm\fontetitretrois#1}\nobreak\smallskip}

% paragraphes de niveaux 4

  \long\def\paraquatre#1{\ifdim\lastskip<\smallskipamount
                \removelastskip\smallskip\fi
                 \vskip0pt plus.01\vsize\penalty-10
                  \vskip0pt
                  plus-.01\vsize\par
                %\bigskip
 
\Indentation{\fontetitrequatre \the\titreun{${\cdot}$}\the\titredeux${\cdot}$\the\titretrois${\cdot}$\incr{\titrequatre}.\ }
{\hskip0mm\fontetitrequatre#1}\nobreak\smallskip}

% paragraphes de niveau 4 numŽrotŽs avec des lettres minuscules


\newtoks\titrequatrel
\titrequatrel={\ifnum\titrequatre=1{a}\fi%
\ifnum\titrequatre=2{b}\fi%
\ifnum\titrequatre=3{c}\fi%
\ifnum\titrequatre=4{d}\fi%
\ifnum\titrequatre=5{e}\fi%
\ifnum\titrequatre=6{f}\fi%
\ifnum\titrequatre=7{g}\fi%
\ifnum\titrequatre=8{h}\fi%
\ifnum\titrequatre=9{i}\fi%
\ifnum\titrequatre=10{j}\fi%
\ifnum\titrequatre=11{k}\fi%
\ifnum\titrequatre=12{l}\fi%
\ifnum\titrequatre=13{m}\fi%
}
\long\def\paraquatrel#1{\ifdim\lastskip<\smallskipamount
                \removelastskip\smallskip\fi
                 \vskip0pt plus.01\vsize\penalty-10
                  \vskip0pt
                  plus-.01\vsize{\bigskip
\Indentation{\global\advance\titrequatre by 1
\fontetitrequatre\quad \quad \quad \the\titreunl${\cdot}$\the\titredeuxl${\cdot}$\the\titretrois${\cdot}$\the\titrequatrel.\ }
{\hskip0mm\fontetitrequatre#1}\nobreak\smallskip}}

% Pour memoriser le no de section d'un titre de paragraphe
\ifx\optionkeys\oui
\def\drefun#1{\definexref{¤#1}{{\the\titreun}}{}} 
\def\drefdeux#1{\definexref{¤#1}{{\the\titreun}.{\the\titredeux}}{}}
\def\dreftrois#1{\definexref{¤#1}{{\the\titreun}.{\the\titredeux}.{\the\titretrois}}{}}
\else
\def\drefun#1{\definexref{prg#1}{{\the\titreun}}{}} 
\def\drefdeux#1{\definexref{prg#1}{{\the\titreun}.{\the\titredeux}}{}}
\def\dreftrois#1{\definexref{prg#1}{{\the\titreun}.{\the\titredeux}.{\the\titretrois}}{}}
\fi

% Dans le cas de \drefun, coder \paraun{Titre}\drefun{label} dans le cas de \drefdeux, on peut coder
%                                \paradeux{Sous-titre\drefdeux{label}}
% pour appeler la reference "label", taper \refn{¤label}
%
% en cas de probl\`emes avec option_keys: coder \def\optionkeys{oui} et remplacer ¤ par prg dans \refn


%% num\'erotation des \'enonc\'es
%%Exemples
%%\propt{leb}{ (Lebesgue)}{ L'espace $L^1$ est complet.}
%%\par
%%Ca marche, comme le dit le \ref{leb}.
%%\Propt{leb2}{L'espace $L^1$ est vraiment complet.}\par
%%Ce \ref{leb2} est moins bien que les Th\'eor\`emes \ref{sleb} et \ref{sleb2}.

  
  \long\def\propdeux#1#2#3#4{%
       \avance{\enonce}
       \leavevmode\edef\temp{#2}%
         \ifx\temp\empty 
          \else
           \definexref{#2}{#1~{\the\titreun.\the\enonce}}{enonces}
            \definexref{s#2}{{\the\titreun.\the\enonce}}{enonces}
             \fi
\smallskip
      \noindent{\bf#1\ {\bf\the\titreun.\the\enonce{#3}.}\enspace}{\sl#4\par}%
      \ifdim\lastskip<\medskipamount \removelastskip\penalty55\par \fi
   }


  \long\def\propun#1#2#3#4{%
      \avance{\enonce}
       \leavevmode\edef\temp{#2}%
        \ifx\temp\empty 
          \else
           \definexref{#2}{#1~{\the\enonce}}{enonces}
            \definexref{{s#2}}{{\the\enonce}}{enonces}
             \fi
   \par 
     \noindent{\bf#1\ {\bf\the\enonce{#3}.}\enspace}{\sl#4\par}%
     \ifdim\lastskip<\medskipamount \removelastskip\penalty55\medskip\fi
  }
  
  \long\def\prop#1#2#3#4{\ifnum\optionparag=1
                          \propdeux{#1}{#2}{\textfont1=\elevenib#3}{#4} \else\propun{#1}{#2}{\textfont1=\elevenib#3}{#4}\fi}
  
 
  \long\def\propt#1#2#3{\ifx\tpf\oui \prop{Th\'eo\-r\`eme}{#1}{#2}{#3}\par
                       \else\prop{Theorem}{#1}{#2}{#3}\par\fi}
  \long\def\Propt#1#2{\propt{#1}{}{#2}}
  \long\def\propl#1#2#3{\ifx\tpf\oui\prop{Lem\-me}{#1}{#2}{#3}\par
                         \else\prop{Lemma}{#1}{#2}{#3}\par\fi}
  \long\def\Propl#1#2{\propl{#1}{}{#2}}
  \long\def\propc#1#2#3{\ifx\tpf\oui\prop{Corol\-laire}{#1}{#2}{#3}\par
                         \else\prop{Corollary}{#1}{#2}{#3}\par\fi}
  \long\def\Propc#1#2{\propc{#1}{}{#2}}
  \long\def\propp#1#2#3{\prop{Pro\-po\-si\-tion}{#1}{#2}{#3}\par}
  \long\def\Propp#1#2{\propp{#1}{}{#2}} 
  \long\def\propd#1#2#3{\ifx\tpf\oui\prop{D\'efi\-nition}{#1}{#2}{#3}\par
                       \else\prop{Definition}{#1}{#2}{#3}\par\fi} 
  \long\def\Propd#1#2{\propd{#1}{}{#2}}
  \long\def\proptd#1#2#3{\ifx\tpf\oui\prop{Th\'eor\`eme et d\'efi\-nition}{#1}{#2}{#3}\par
                       \else\prop{Theorem and definition}{#1}{#2}{#3}\par\fi} 
  \long\def\Proptd#1#2{\proptd{#1}{}{#2}}

  % Pour une numerotation des enonces et des formules avec un seul nombre 
  % coder \optionparag=2

  % Choisir numerotation manuelle ou automatique des paragraphes: 
  % utiliser \section au lieu de \paraun et choisir \optionparag=2
  % Cela induit aussi une num\'erotation des formules avec un seul nombre
  
  \newcount\optionparag\optionparag=1
  
  \long\def\section#1#2{\ifnum\optionparag=1 \paraun{#2} 
                        \else\goodbreak{\fontetitreun
  	                \Indentation{#1.\ }{#2}}\nobreak\smallskip\fi}
 
  
  \long\def\sectionl{\section}
  
  \def\numauto{\optionparag=1}  % numerotation automatique (par defaut)
  \def\nummanu{\optionparag=2}  % numerotation manuelle
  \def\eqconstruct#1{\ifnum\optionparag=1{\the\titreun\hbox{$\cdot$}#1}\else{#1}\fi}
  \def\eqprint#1{{\rm (#1)}}
  
  
  %%%%%%% Fin num\'erotation automatique des paragraphes
  
  %% num\'erotation bibliographie
  
  \def\numref{oui}  % numeroter la biblio par defaut avec bibtem
  
  \newcount\mesref\mesref=0 
  \def\defbib#1{\ifx\numref\oui\global\advance\mesref by 1 \definexref{#1}{{\the
                 \mesref}}{}\else\definexref{#1}{#1}{}\fi}
  \def\bibtem#1{\defbib{#1}\item{\citer{#1}}}
  \def\citer#1{[\ref{#1}]}
  \def\citeplus#1#2{[\ref{#1}; #2]}
  
  
  
  % FONTES & FAMILLES
  
  \font\seventeenmsa=msam10 at 17pt    % symboles d'AMSTEX
  \font\fourteenmsa=msam10 at 14pt
  \font\twelvemsa=msam10 at 12pt
  \font\tenmsa=msam10                 
  \font\ninemsa=msam10 at 9pt 
  \font\eightmsa=msam10 at 8pt 
  \font\sevenmsa=msam7 
  \font\sixmsa=msam10 at 6pt
  \font\fivemsa=msam5
  \newfam\msafam\textfont\msafam=\tenmsa\scriptfont\msafam=\sevenmsa\scriptscriptfont\msafam=\fivemsa
  
  \font\seventeenbb=msbm10 at 17pt     % Lettres evidees pour titres
  \font\fourteenbb=msbm10 at 14pt
  \font\twelvebb=msbm10 at 12pt
  \font\tenbb=msbm10                   %Lettres evidees
  \font\ninebb=msbm10 at 9pt 
  \font\eightbb=msbm10 at 8pt 
  \font\sevenbb=msbm7 
  \font\sixbb=msbm10 at 6pt
  \font\fivebb=msbm5 
  \newfam\bbfam\textfont\bbfam=\tenbb\scriptfont\bbfam=\sevenbb\scriptscriptfont\bbfam=\fivebb
  \def\bb{\fam\bbfam\tenbb}%
  
  
  \font\seventeenscaln=eusm10 at 17pt   % Lettres de ronde
  \font\twelvescaln=eusm10 at 12pt
  \font\tenscaln=eusm10                
  \font\ninescaln=eusm10 scaled 900
  \font\eightscaln=eusm10 scaled 800
  \font\sevenscaln=eusm10 scaled 700
  \font\sixscaln=eusm10 scaled 600
  \font\fivescaln=eusm5 
  \newfam\scalnfam\textfont\scalnfam=\tenscaln\scriptfont\scalnfam=\sevenscaln\scriptscriptfont\scalnfam=\sixscaln
  \def\scaln{\fam\scalnfam\tenscaln}%
  \def\scal{\scaln}
  
  \font\tenscalb=eusb10                % Lettres de ronde grasses
  \font\ninescalb=eusb10 scaled 900
  \font\eightscalb=eusb10 scaled 800
  \font\sevenscalb=eusb10 scaled 700
  \font\sixscalb=eusb10 scaled 600
  \font\fivescalb=eusb5 
  \newfam\scalbfam\textfont\scalbfam=\tenscalb\scriptfont\scalbfam=\sevenscalb
  \def\scalb{\fam\scalbfam\tenscalb}%
  
  %
  % Romain
  %
  \font\fourteenrm=cmr12 scaled 1200
  \font\elevenrm=cmr10 at 11pt
  \font\twelverm=cmr12
  \font\ninerm=cmr9
  \font\eightrm=cmr8      
  \font\sevenrm=cmr7
  \font\sixrm=cmr6
  
  
  \font\seventeenpcap=cmcsc10 at 17pt
  \font\tenpcap=cmcsc10                        % Petites capitales
  \font\ninepcap=cmcsc9
  \font\eightpcap=cmcsc8
  \font\sevenpcap=cmcsc10 scaled 700
  \font\sixpcap=cmcsc10 scaled 600
  \newfam\pcapfam\textfont\pcapfam=\tenpcap\scriptfont\pcapfam=\sevenpcap
  \def\pcap{\fam\pcapfam\tenpcap}
  
  \font\gras=cmbx10 scaled 1100             % Gras romain (boldface)
  \font\TIT=cmbx12 scaled 1600              % Titres
  \font\seventeenrm=cmbx12 scaled 1400
  \font\chiffre=cmbx10 scaled 1600
  \font\titre=cmbx12 scaled 1200
  \font\pti=cmbx12 scaled 1200
  \font\sixteenbf=cmbx10 at 16 pt
  \font\fourteenbf=cmbx10 scaled 1400
  \font\thirteenbf=cmbx10 at 13pt
  \font\twelvebf=cmbx12
  \font\elevenbf=cmbx10 at 11pt
  \font\ninebf=cmbx9  
  \font\eightbf=cmbx8
  \font\sixbf=cmbx6
  
  \font\tengot=eufm10                           % Lettres gothiques
  \font\ninegot=eufm10 at 9pt 
  \font\eightgot=eufm10 at 8truept 
  \font\sevengot=eufm7 
  \font\sixgot=eufm10 at 6 truept 
  \font\fivegot=eufm5 
  \newfam\gotfam
  \textfont\gotfam=\tengot\scriptfont\gotfam=\sevengot\scriptscriptfont\gotfam=\sixgot
  \def\got{\fam\gotfam\tengot}%
  
  
  %% Pour les titres (168pt)
  
  \def\tit{%
  \textfont0=\seventeenrm\scriptfont0=\tenrm\def\rm{\fam0\seventeenrm}%
  \textfont1=\seventeenib\scriptfont1=\twelveib%
  \textfont2=\seventeensy\scriptfont2=\twelvesy\scriptscriptfont2=\ninesy
  \textfont3=\seventeenex
  \textfont\itfam=\seventeenti
  \def\it{\fam\itfam\seventeenti}%
  \textfont\bbfam=\seventeenbb \scriptfont\bbfam=\twelvebb
  \def\bb{\fam\bbfam\seventeenbb}%
  \textfont\msafam=\seventeenmsa\scriptfont\msafam=\twelvemsa
  \textfont\scalnfam=\seventeenscaln
  \def\pcap{\fam\pcapfam\seventeenpcap}
  \normalbaselineskip=25pt\normalbaselines\rm}
  
  
  % italiques grasses pour titres
  \font\seventeenti=cmbxti10 scaled 1680
  \font\sixteenti=cmbxti10 scaled 1600
  \font\fourteenti=cmbxti10 at 14pt
  \font\thirteenti=cmbxti10 at 13pt
  \font\twelveti=cmbxti10 scaled 1200
  \font\eleventi=cmbxti10 at 11pt
  \font\tenti=cmbxti10
  \font\nineti=cmbxti10 at 9pt
  \font\seventi=cmbxti10 at 7pt
  
  %
  % italiques
  %
  \font\twelveit=cmti12	
  \font\elevenit=cmti10 scaled 1100
  \font\nineit=cmti9
  \font\eightit=cmti8
  \font\sevenit=cmti7
  \font\sixit=cmti10 scaled 600              			  
  \font\fiveit=cmti10 scaled 500
  
  %
  % italique mathematique gras pour titres
  %
 
 \font\seventeenib=cmmib10 scaled 1680
  \font\fourteenib=cmmib10 scaled 1400
  \font\twelveib=cmmib10 scaled 1200
  \font\elevenib=cmmib10 scaled 1100
  \font\tenib=cmmib10
\font\eightib=cmmib10 scaled 800
  \font\nineib=cmmib10 scaled 900
\font\sevenib=cmmib10 scaled 700
\font\sixib=cmmib10 scaled 600
\font\fiveib=cmmib10 scaled 500

\ifx\ITAN\oui
\else
\innernewfam\cmmibfam
\textfont\cmmibfam=\tenib
\scriptfont\cmmibfam=\sevenib
\scriptscriptfont\cmmibfam=\fiveib
\def\ib{\fam\cmmibfam\tenib}
\fi

  %
  % italique mathematique
  %
  \font\twelvei=cmmi10 scaled 1200
  \font\eleveni=cmmi10 scaled 1100
  \font\ninei=cmmi9
  \font\eighti=cmmi8 
  \font\seveni=cmmi7 			                
  \font\sixi=cmmi6
  
  \font\ninesl=cmsl9                    % slanted 
  \font\eightsl=cmsl8 
  \font\sevensl=cmsl10 at 7pt
  \font\sixsl=cmsl10 at 6pt                  
  \font\fivesl=cmsl10 at 5pt
  
  \font\ninett=cmtt9                    % typewriter
  \font\eighttt=cmtt8
  \font\seventt=cmtt10 scaled 700
  \font\sixtt=cmtt10 scaled 550
  \font\fivett=cmtt10 scaled 500
  
  \font\seventeensy=cmsy10 scaled 1680    % symboles pour titres
  \font\fourteensy=cmsy10 scaled 1400
  \font\twelvesy=cmsy10 scaled 1176
  \font\elevensy=cmsy10 scaled 1100
  \font\ninesy=cmsy9                      % symboles
  \font\eightsy=cmsy8
  \font\sixsy=cmsy6
  \font\seventeenex=cmex10 at 17pt
  \font\fourteenex=cmex10 at 14pt
  \font\twelveex=cmex10 at 12pt
  \font\nineex=cmex10 at 9pt
  \font\eightex=cmex10 at 8pt
  \font\sevenex=cmex10 at 7pt
  \font\sixex=cmex10 at 6pt
  \font\fiveex=cmex10 at 5pt
  
   %% Lettres grecques plombees              %% Lettres grecques plombees
   
  \font\fourteengp=cmmi10 at 14pt
  \font\thirteengp=cmmib10 at 13pt
  \font\twelvegp=cmmib10 at 12pt
  \font\elevengp=cmmib10 at 11pt
  \font\tengp=cmmib10                          
  \font\ninegp=cmmib10 at 9pt 
  \font\eightgp=cmmib8 
  \font\sevengp=cmmib7 
  \font\sixgp=cmmib6
  \font\fivegp=cmmib5 

%\innernewfam\gpfam
%\textfont1\gpfam=\tengp
%\scriptfont1\gpfam=\sevengp
%\scriptscriptfont1\gpfam=\fivegp
%\def\gp{\fam\gpfam\tengp}
 
\def\gpsept{\textfont0=\sevenbf\scriptfont0=\sixbf\scriptscriptfont0=\fivebf
           \textfont1=\sevengp\scriptfont1=\sixgp\scriptscriptfont1=\fivegp}

 \def\gphuit{\textfont0=\eightbf\scriptfont0=\sixbf\scriptscriptfont0=\fivebf
           \textfont1=\eightgp\scriptfont1=\sixgp\scriptscriptfont1=\fivegp}
\def\gp{\textfont0=\tenbf\scriptfont0=\sevenbf\scriptscriptfont0=\fivebf
\textfont1=\tengp\scriptfont1=\sevengp\scriptscriptfont1=\fivegp}
  \def\gponze{\textfont0=\elevenbf\scriptfont0=\eightbf\scriptscriptfont0=\sixbf
           \textfont1=\elevengp\scriptfont1=\eightgp\scriptscriptfont1=\sixgp}
  \def\gpdouze{\textfont0=\twelvebf\scriptfont0=\tenbf\scriptscriptfont0=\ninebf
           \textfont1=\twelvegp\scriptfont1=\tengp\scriptscriptfont1=\ninegp}        
  \def\gptreize{\textfont0=\thirteenbf\scriptfont0=\elevenbf\scriptscriptfont0=\tenbf
           \textfont1=\thirteengp\scriptfont1=\elevengp\scriptscriptfont1=\tengp}
 \def\gpquatorze{\textfont0=\fourteenbf\scriptfont0=\twelvebf\scriptscriptfont0=\elevenbf
           \textfont1=\fourteengp\scriptfont1=\twelvegp\scriptscriptfont1=\elevengp}
  
  
  % CARACTERES SPECIAUX
  
  \expandafter\chardef\csname pre amssym.def at\endcsname=\the\catcode`\@
  \catcode`\@=11
  \def\undefine#1{\let#1\undefined}
  \def\newsymbol#1#2#3#4#5{\let\next@\relax
   \ifnum#2=\@ne\let\next@\msafam@\else
   \ifnum#2=\tw@\let\next@\bbfam@\fi\fi
   \mathchardef#1="#3\next@#4#5}
  \def\mathhexbox@#1#2#3{\relax
   \ifmmode\mathpalette{}{\m@th\mathchar"#1#2#3}%
   \else\leavevmode\hbox{$\m@th\mathchar"#1#2#3$}\fi}
  \def\hexnumber@#1{\ifcase#1 0\or 1\or 2\or 3\or 4\or 5\or 6\or 7\or 8\or
   9\or A\or B\or C\or D\or E\or F\fi}
  
  \def\setboxz@h{\setbox\z@\hbox}
  \def\wdz@{\wd\z@}
  \def\boxz@{\box\z@}
  
  \edef\msafam@{\hexnumber@\msafam}
  \mathchardef\dabar@"0\msafam@39
  
  \edef\bbfam@{\hexnumber@\bbfam}
  \def\widehat#1{\setboxz@h{$\m@th#1$}%
   \ifdim\wdz@>\tw@ em\mathaccent"0\bbfam@5B{#1}%
   \else\mathaccent"0362{#1}\fi}
  \def\widetilde#1{\setboxz@h{$\m@th#1$}%
   \ifdim\wdz@>\tw@ em\mathaccent"0\bbfam@5D{#1}%
   \else\mathaccent"0365{#1}\fi}
  \newsymbol\leqq 1335          % superieur ou egal(=)
  \newsymbol\leqslant 1336
  \newsymbol\lessgtr 1337       % superieur ou inferieur
  \newsymbol\backprime 1038     % apostrophe de gauche a droite
  \newsymbol\risingdotseq 133A  % egal entre points (bas puis haut)
  \newsymbol\fallingdotseq 133B % egal entre points (haut puis bas)
  \newsymbol\succcurlyeq 133C   % superieur ou egal tordu
  \newsymbol\geqq 133D          % inferieur ou egal(=)
  \newsymbol\geqslant 133E
  \newsymbol\nmid 232D
  \newsymbol\nexists 2040
  \newsymbol\smallsetminus 2272
  \newsymbol\varnothing 203F 
  \catcode`\@=\active
  
 
  \def\nparallel{\mathop{\hbox{\tenbb\char44}}\nolimits}
  
  % typographie francaise ou anglaise
  \catcode`\@=11
  \newcount\typofr\typofr=1
  
  \catcode`\;=\active
  \def;{\ifnum\typofr=1\relax\ifhmode\ifdim\lastskip>\z@\unskip\fi
     \kern.2em\fi\string;\else\string;\fi}
  
  \catcode`\:=\active
  \def:{\ifnum\typofr=1\relax\ifhmode\ifdim\lastskip>\z@\unskip\fi
  \penalty\@M\ \fi\string:\else\string:\fi}
  
  \catcode`\!=\active
  \def!{\ifnum\typofr=1\relax\ifhmode\ifdim\lastskip>\z@\unskip\fi
     \kern.2em\fi\string!\else\string!\fi}
  
  \catcode`\?=\active
  \def?{\ifnum\typofr=1\relax\ifhmode\ifdim\lastskip>\z@\unskip\fi
     \kern.2em\fi\string?\else\string?\fi}
  
  
  \def\francais{\typofr=1\def\tpf{oui}}
  \def\anglais{\typofr=2\def\tpf{non}\def\english{oui}}
  \def\oui{oui}
  \francais
  
  \catcode`\@=12
  %\catcode`\@=\active
  
  %pour rayer du texte en rouge

\ifx\textures\oui
\def\raye #1|{\leavevmode\setbox1=\hbox{#1}%
\raise .5pt\hbox to \wd1{\xleaders\hbox{\rge{$ \sct / $}%
\kern 1pt}\hfill\kern -1pt }\kern -\wd1 \unhbox1\relax }

\def\barre #1|{\leavevmode\setbox1=\hbox{#1}%
\rlap{\Red\vrule height 2.4pt depth -1.2pt width \wd1}\Black \unhbox1\relax}
\else
\def\raye #1|{\leavevmode\setbox1=\hbox{#1}%
\raise .5pt\hbox to \wd1{\xleaders\hbox{\rge{$ \sct / $}%
\kern 1pt}\hfill\kern -1pt }\kern -\wd1 \unhbox1\relax }

\def\barre #1|{\leavevmode\setbox1=\hbox{#1}%
\rlap{\color{red}\vrule height 2.4pt depth -1.2pt width \wd1}\color{black} \unhbox1\relax}

\fi
  
  % FIN CARACTERES SPECIAUX
  
  
  % MACROS DIVERSES
  
  \def\og{\leavevmode\raise.24ex\hbox{$\scriptscriptstyle\langle\!\langle\>$}}    % guillemets ouvrants
  \def\fg{\leavevmode\raise.24ex\hbox{$\scriptscriptstyle\>\rangle\!\rangle$}}    % guillemets fermants
  \def\chv#1{\left\langle#1\right\rangle}
  \def\pchv#1{\langle#1\rangle}
  \def\bchv#1{\big\langle#1\big\rangle}
  \def\d{\,{\rm d}}
  \def\dd{{\rm d}}
  \def\dt{\d t}
  \def\du{\d u}
  \def\dx{\d x}
  \def\dy{\d y}
  \def\z{{\bb Z}}
  \def\r{{\bb R}}
  \def\CC{{\bb C}}
  \def\N{{\bb N}}
  \def\Q{{\bb Q}}
  \def\F{{\bb F}}
  \def\PP{{\bb P}}
  \def\TT{{\bb T}}
  \def\UU{{\bb U}}
  
  \def\A{{\scal A}}
  \def\B{{\scal B}}
  \def\C{{\scaln C}}
  \def\D{{\scal D}}
  \def\E{{\scal E}}
  \def\G{{\scal G}}
  \def\HH{{\scal H}}
  \def\I{{\scal I}}
  \def\J{{\scal J}}
  \def\K{{\scal K}}
  \let\LL=\L
  \def\L{{\scal L}}
  \def\M{{\scal M}}
  \def\n{{\scal N}}
  \def\O{{\scal O}}
  \def\P{{\scaln P}}
  \def\QQ{{\scaln Q}}
  \def\R{{\scal R}}
  \def\s{{\cal S}}
  \def\T{{\scal T}}
  \def\V{{\scal V}}
  \def\W{{\scal W}}
  \def\X{{\scal X}}
  \def\Y{{\scal Y}}
  \def\Z{{\scal Z}}
  \def\f{{\scal F}}
  \def\frac#1#2{{#1\over #2}}
  \def\di#1#2{\sct#1\atop{\sct#2}}
  \def\tri#1#2#3{{\sct#1\atop\sct#2}\atop\sct#3}
 \def\qri#1#2#3#4{{\sct#1\atop\sct#2}\atop{\sct#3\atop\sct#4}}
  \def\wt{\widetilde}
  \def\numero{n$^{\rm o}\thinspace$}
\def\numeros{n$^{\rm os}\thinspace$}
  \def\page#1{\rm p.\thinspace#1}
  \def\theoreme#1{\rm th.\thinspace#1}
  \def\chapitre#1{\rm chap.\thinspace#1}
  \def\qedbox{$\rlap{$\sqcap$}\sqcup$}           % carr\'e blanc fin de d\'emo
  \def\qed{\nobreak\hfill\penalty250 \hbox{}\nobreak\hfill\qedbox\par }
  \def\Ssi{si, et seulement si, }
  \def\CN{condition n\'ecessaire}
  \def\cn{\CN}
  \def\CS{condition suffisante}
  \def\CNS{condition n\'ecessaire et suffisante}
  \def\cns{\CNS}
  \def\fa{fonc\-tion arith\-m\'etique}
  \def\fas{fonc\-tions arith\-m\'etiques}
  \def\HR{hypoth\`ese de Riemann}
  \def\leg#1#2{\({#1\over #2}\)}
  \def\sD{s\'erie de Dirichlet}
  \def\sDS{s\'eries de Dirichlet}
  \def\sumast{\mathop{{\sum}^*}}
  \def\sumdast{\mathop{{\sum}^{**}}}
  \def\numero{n$^{\rm o}\thinspace$}
  \def\np{nombre premier}
  \def\nps{nombres premiers}
  \def\tnp{th\'eo\-r\`eme des nombres premiers}
  \def\TNP{\tnp}
  \def\pnu{p^\nu}
  \def\thm{th\'eo\-r\`eme}
  \def\pnt{prime number theorem}
  \def\TAN{th\'eorie analytique des nombres}
  \def\TL{transform\'ee de Laplace}
  \def\TF{transform\'ee de Fourier}
  \def\TFs{transform\'ees de Fourier}
  \def\plaf#1{\left\lceil#1\right\rceil}
  \def\planch#1{\left\lfloor#1\right\rfloor}
  \def\¤{\S\thinspace}
  \def\prt#1{\left(#1\right)}
  \def\Prt#1{\Big(#1\Big)}
  %\def\jetdencre{\input CrayolaColors\vskip4cm\White mise en page\Black}
  \def\¥{$\bullet$ }
  
  %SYMBOLES MATHS
  
  \def\e{{\rm e}}
  \def\mod{\mathop{\rm mod}\nolimits}
  \def\md#1#2{\equiv#1\,({\rm mod\,}#2)}
  \def\no#1{\Vert#1\Vert}
  \def\No#1{\Big\Vert#1\Big\Vert}
  \def\NO#1{\left\Vert#1\right\Vert}
  \def\ddp#1#2{\dsp{\partial#1\over\partial #2}}
  \def\ent#1{\left[#1\right]}
  \def\tdv{\rightarrow}
  \def\ssi{\Leftrightarrow}
  \def\tvi{\tdv +\infty}
  %\def\v{\varepsilon}
  \def\exemple{\par\noi{\it Exemple. }}
  \def\exemples{\par\noi{\it Exemples. }}
  \def\exercice{\par\noi{\it Exercice. }}
  \def\exercices{\par\noi{\it Exercices. }}
  \def\ep{\varepsilon}
  \def\epsilon{\varepsilon}
  \def\om{\omega}
  \def\Om{\Omega}
  \let\oldphi=\phi
  \def\phi{\varphi}
  \def\theta{\vartheta}
  \def\rho{\varrho}
  \def\dm{{\textstyle{1\over 2}}}
  \def\txt{\textstyle}
  \def\dsp{\displaystyle}
  \def\sct{\scriptstyle}
  \def\pf{\noi{\it Proof. }}
  \def\nid{\ifnum\typofr=1\par\noindent{\it D\'emonstration. }\else\pf\fi}
  \def\noi{\noindent}
  \def\rem{\ifnum\typofr=1\noi{\it Remarque.}\ \else\noi{\it Remark.}\ \fi}
  \def\rems{\ifnum\typofr=1\noi{\it Remarques.}\ \else\noi{\it Remarks.}\ \fi}
  \def\re{{\Re e\,}}
  \def\im{{\Im m\,}}
  \def\ov{\overline}
  \def\un{\underline}
  \def\sset{\smallsetminus}
  \def\setminus{\sset}
  \def\emptyset{{\varnothing}}
  \def\pl{\partial}
  \def\pp{{\rm pp}}
  \def\det{\mathop{\hbox{\rm d\'et}}\nolimits}
  \def\meas{\mathop{\rm meas}\nolimits}
  \def\dim{\mathop{\rm dim}\nolimits}
  \def\1{{\bf 1}}
  \def\|{\Vert}
  \let\vieuxle=\le
  \let\vieuxge=\ge
  \def\le{\leqslant}\def\leq{\leqslant}
  \def\ge{\geqslant}\def\geq{\geqslant}
  \def\wh{\widehat}
  \def\cf{{cf.}}
  \def\ie{{i.e.\ }}
  \def\eg{{e.g.}}
  \newsymbol\subsetneqq 2324
  \newsymbol\subsetneq 2328
  %% operateurs
  
  \def\card{\mathop{\rm card}\nolimits}
  \def\sh{\mathop{\rm sh}\nolimits}
  \def\th{\mathop{\rm th}\nolimits}
  \def\tg{\mathop{\rm tg}\nolimits}
  \def\arctg{\mathop{\rm arctg}\nolimits}
  \def\arccotg{\mathop{\rm arccotg}\nolimits}
  \def\arcsin{\mathop{\rm arcsin}\nolimits}
  \def\arccos{\mathop{\rm arccos}\nolimits}
  \def\argth{\mathop{\rm argth}\nolimits}
  \def\ch{\mathop{\rm ch}\nolimits}
  \def\Ker{\mathop{\rm Ker}\nolimits}
  \def\fl#1{\left\lfloor #1 \right\rfloor}
  \def\plaf#1{\left\lceil #1 \right\rceil}
   \def\fll#1{\big\lfloor #1 \big\rfloor}
  \def\plafl#1{\big\lceil #1 \big\rceil}
  \def\li{\mathop{\rm li}\nolimits}
  \def\sgn{\mathop{\rm sgn}\nolimits}
  \def\supp{\mathop{\rm supp}\nolimits}
  \def\grad{\mathop{\rm grad}\nolimits}
  \def\log{\mathop{\rm log}\nolimits}
  \def\ft#1#2{{\txt{#1\over #2}}}
  \def\fs#1#2{{\scriptstyle{#1\over #2}}}
  \def\sumstar{\mathop{{\sum}^*}}
  %% Grande asterisque operateur
  \font\gm=cmbx10 scaled 2000
  \def\bst{\smash{\atop\hbox{\gm *}}}
  \def\gast#1#2{\mathop{\bst}_{\phantom A \atop{\sct #1}}#2}
  %% Grande asterisque sur la ligne
  \def\glast#1#2{\mathop{\bst}_{\atop\sct #1}#2}
\def\vbs#1{\left|#1\right|}
\def\Vbs#1{\bigg|#1\bigg|}
\def\abs#1{\left|#1\right|}

  
  
  %fleches
  
  \def\gradv{\mathop{\overrightarrow{\rm grad}}\nolimits}
  \def\vec{\overrightarrow}
  
  
  %% Lettres plombees 'pauvres'
  \def\pmb#1{\setbox0=\hbox{#1}%
  \kern-.025em\copy0\kern-\wd0\kern.05em\copy0\kern-\wd0\kern-.025em\raise .0433em\box0 }
  \def\pd{\pmb{$\delta$}}
  
  
  % NOTES EN BAS DE PAGE
  
  % Pour que les accents se placent correctement en mode math en corps 8 et 6
  \skewchar\eighti='177 \skewchar\sixi='177
  \skewchar\eightsy='60 \skewchar\sixsy='60
  
  \def\eightpoint{%
  \textfont0=\eightrm\scriptfont0=\sixrm\scriptscriptfont0=\fiverm
  \def\rm{\fam0\eightrm}%
  \textfont1=\eighti\scriptfont1=\sixi
  \scriptscriptfont1=\fivei\def\oldstyle{\fam1\seveni}%
  \textfont2=\eightsy\scriptfont2=\sixsy\scriptscriptfont2=\fivesy
  \textfont3=\eightex\scriptfont3=\sixex
  \textfont\itfam=\eightit
  \def\it{\fam\itfam\eightit}%
  \textfont\slfam=\eightsl
  \def\sl{\fam\slfam\eightsl}%
  \textfont\bbfam=\eightbb \scriptfont\bbfam=\sixbb\scriptscriptfont\bbfam=\fivebb
  \def\bb{\fam\bbfam\eightbb}%
  \textfont\msafam=\eightmsa\scriptfont\msafam=\sixmsa
  \textfont\scalnfam=\eightscaln
  \def\scaln{\fam\scalnfam\eightscaln}
  \textfont\ttfam=\eighttt
  \def\tt{\fam\ttfam\eighttt}%
\textfont\gotfam=\eightgot
  \textfont\bffam=\eightbf\scriptfont\bffam=\sixbf\scriptscriptfont\bffam=\fivebf
  \def\bf{\fam\bffam\eightbf}%
  \ifx\ITAN\oui\else\textfont\cmmibfam=\eightib
       \scriptfont\cmmibfam=\sixib
        \scriptscriptfont\cmmibfam=\fiveib
         \def\ib{\fam\cmmibfam\eightib}
   \fi
  \textfont\pcapfam=\eightpcap
  \def\pcap{\fam\pcapfam\eightpcap}
  \abovedisplayskip=2pt plus2pt minus 2pt
  \belowdisplayskip=2pt plus1pt minus 2pt
  \abovedisplayshortskip= 1pt plus 2pt minus 1pt
  \belowdisplayshortskip= 1pt plus 2pt minus 1pt
  \smallskipamount=2pt plus 1pt minus 2pt
  \medskipamount=3pt plus 2pt minus 2pt
  \bigskipamount=7pt plus 3pt minus 3pt
  \setbox\strutbox=\hbox{\vrule height 5pt depth 2pt width 0pt}%
  \normalbaselineskip=9pt\normalbaselines\rm}
  
  
  %\def\note#1#2{\footnote{#1}{\noi\eightpoint #2\vskip-10pt\par}}
  %\def\note#1#2{\hbox{$^{(#1)}$}\footnote{}{\eightpoint$#1.$  #2\vskip-10pt\par}}
  \def\pclm#1#2{\noi\bf#1\sl\ #2}
  
  \def\({\left(}
  \def\){\right)}
  
  \def\footnoterule{\kern -2pt\hrule width 7truecm\kern 2.4pt}
  
  %reference croisee a des numeros de notes
  \def\xnotedef#1{\definexref{#1}{\noexpand\number\footnotenumber}{Note}}%
  \def\noteref{\ref}
  
  %Fin des definitions pour les notes en bas de page
  
  % PARAGRAPHES EN NEUF POINTS
  
  \def\ninepoint{%
  \textfont0=\ninerm\scriptfont0=\sixrm\scriptscriptfont0=\fiverm
  \def\rm{\fam0\ninerm}%
  \textfont1=\ninei\scriptfont1=\sixi
  \scriptscriptfont1=\fivei\def\oldstyle{\fam1\ninei}%
  \textfont2=\ninesy\scriptfont2=\sixsy\scriptscriptfont2=\fivesy
  \textfont3=\nineex\scriptfont3=\sixex
  \textfont\itfam=\nineit
  \def\it{\fam\itfam\nineit}%
  \textfont\slfam=\ninesl
  \def\sl{\fam\slfam\ninesl}%
  \textfont\bbfam=\ninebb\scriptfont\bbfam=\sixbb\scriptscriptfont\bbfam=\fivebb
  \def\bb{\fam\bbfam\ninebb}%
  \textfont\msafam=\ninemsa\scriptfont\msafam=\sixmsa\scriptscriptfont\msafam=\fivemsa
  \textfont\scalnfam=\ninescaln
  \def\scaln{\fam\scalnfam\ninescaln}
  \textfont\ttfam=\ninett
  \def\tt{\fam\ttfam\ninett}%
  \textfont\bffam=\ninebf\scriptfont\bffam=\sixbf\scriptscriptfont\bffam=\fivebf
  \def\bf{\fam\bffam\ninebf}%
  \abovedisplayskip=3pt plus2pt minus 2pt
  \belowdisplayskip=3pt plus1pt minus 2pt
  \abovedisplayshortskip= 2pt plus 2pt minus 1pt
  \belowdisplayshortskip= 2pt plus 2pt minus 1pt
  \smallskipamount=2pt plus 1pt minus 2pt
  \medskipamount=3pt plus 2pt minus 2pt
  \bigskipamount=7pt plus 3pt minus 3pt
  \setbox\strutbox=\hbox{\vrule height 5pt depth 2pt width 0pt}%
  \normalbaselineskip=11pt plus.3pt minus.2pt\normalbaselines\rm}
  
  \def\neufpts#1{{\ninepoint#1}\par}
  
  \def\sevenpoint{%
  \textfont0=\sevenrm\scriptfont0=\sixrm\scriptscriptfont0=\fiverm
  \def\rm{\fam0\sevenrm}%
  \textfont1=\seveni\scriptfont1=\sixi
  \scriptscriptfont1=\fivei\def\oldstyle{\fam1\seveni}%
  \textfont2=\sevensy\scriptfont2=\sixsy\scriptscriptfont2=\fivesy
  \textfont3=\sevenex\scriptfont3=\fiveex
  \textfont\itfam=\sevenit
  \def\it{\fam\itfam\sevenit}%
  \textfont\slfam=\sevensl
  \def\sl{\fam\slfam\sevensl}%
  \textfont\bbfam=\sevenbb \scriptfont\bbfam=\sixbb\scriptscriptfont\bbfam=\fivebb
  \def\bb{\fam\bbfam\sevenbb}%
  \textfont\msafam=\sevenmsa\scriptfont\msafam=\sixmsa
  \textfont\scalnfam=\sevenscaln
  \def\scaln{\fam\scalnfam\sevenscaln}
  \textfont\bffam=\sevenbf\scriptfont\bffam=\sixbf\scriptscriptfont\bffam=\fivebf
  \def\bf{\fam\bffam\sevenbf}%
  \textfont\ttfam=\seventt
  \abovedisplayskip=2pt plus2pt minus 2pt
  \belowdisplayskip=2pt plus1pt minus 2pt
  \abovedisplayshortskip= 1pt plus 2pt minus 1pt
  \belowdisplayshortskip= 1pt plus 2pt minus 1pt
  \smallskipamount=2pt plus 1pt minus 2pt
  \medskipamount=3pt plus 2pt minus 2pt
  \bigskipamount=7pt plus 3pt minus 3pt
  \setbox\strutbox=\hbox{\vrule height 5pt depth 2pt width 0pt}%
  \normalbaselineskip=9pt\normalbaselines\rm}
  
\def\dixpts{%
 \textfont0=\tenrm\scriptfont0=\eightrm\scriptscriptfont0=\sixrm
 \def\rm{\fam0\tenrm}
 \textfont1=\teni\scriptfont1=\eighti\scriptscriptfont1=\sixi
\textfont2=\tensy\scriptfont2=\sevensy\scriptscriptfont2=\sixsy
\textfont3=\tenex\scriptfont3=\sevenex
\textfont\itfam=\tenit \def\it{\fam\itfam\tenit}%
\textfont\slfam=\tensl \def\sl{\fam\slfam\tensl}%
\textfont\ttfam=\tentt \def\tt{\fam\ttfam\tentt}%
\textfont\bffam=\tenbf\scriptfont\bffam=\sevenbf\scriptscriptfont\bffam=\fivebf
 \def\bf{\fam\bffam\tenbf}%
\textfont\gotfam=\tengot\scriptfont\gotfam=\sevengot\scriptscriptfont\gotfam=\fivegot
 \def\got{\fam\gotfam\tengot}%
\textfont\bbfam=\tenbb\scriptfont\bbfam=\sevenbb\scriptscriptfont\bbfam=\fivebb
 \def\bb{\fam\bbfam\tenbb}%
 \abovedisplayskip=11pt plus2pt minus 7pt
  \belowdisplayskip=11pt plus2pt minus 7pt
  \abovedisplayshortskip= 1pt plus 2pt minus 1pt
  \belowdisplayshortskip= 2pt plus 1pt minus 1pt
  \smallskipamount=2pt plus 1pt minus 2pt
  \medskipamount=6pt plus 2pt minus 2pt
  \bigskipamount=11pt plus 3pt minus 4pt
\normalbaselineskip=12.5pt plus.4pt minus.3pt\normalbaselines
\rm}

 \def\onzepts{%
 \textfont0=\elevenrm\scriptfont0=\ninerm
 \textfont1=\eleveni\scriptfont1=\ninei
}

\def\douzepts{%
  \textfont0=\twelverm\scriptfont0=\tenrm\def\rm{\fam0\twelverm}%
  \textfont1=\twelvei\scriptfont1=\teni%
  \textfont2=\twelvesy\scriptfont2=\tensy\scriptscriptfont2=\eightsy
  \textfont3=\twelveex
  \textfont\itfam=\twelveti
  \def\it{\fam\itfam\twelveti}%
  \textfont\bffam=\twelvebf\scriptfont\bffam=\tenbf\scriptscriptfont\bffam=\eightbf
  \def\bf{\fam\bffam\twelvebf}%
  \textfont\bbfam=\twelvebb \scriptfont\bbfam=\tenbb
  \def\bb{\fam\bbfam\twelvebb}%
  \textfont\msafam=\twelvemsa\scriptfont\msafam=\tenmsa
  \textfont\scalnfam=\twelvescaln
  \normalbaselineskip=15pt\normalbaselines\rm}

\def\quatorzepts{%
  \textfont0=\fourteenrm\scriptfont0=\twelverm\def\rm{\fam0\fourteenrm}%
  \textfont1=\fourteenib\scriptfont1=\twelveib%
  \textfont2=\fourteensy\scriptfont2=\twelvesy\scriptscriptfont2=\tensy
  \textfont3=\fourteenex
  \textfont\itfam=\fourteenti
  \def\it{\fam\itfam\fourteenti}%
  \textfont\bffam=\fourteenbf\scriptfont\bffam=\twelvebf\scriptscriptfont\bffam=\tenbf
  \def\bf{\fam\bffam\fourteenbf}%
  \textfont\bbfam=\fourteenbb \scriptfont\bbfam=\twelvebb
  \def\bb{\fam\bbfam\fourteenbb}%
  \textfont\msafam=\fourteenmsa\scriptfont\msafam=\twelvemsa
  \textfont\scalnfam=\twelvescaln
  \normalbaselineskip=18pt\normalbaselines\rm}


% Bibliographies, journaux

\def\AA{{\it Acta Arith.}}
\def\BSMF{{\it Bull. Soc. Math. France}}
\def\Crelle{{\it J. reine angew. Math.}}
\def\JLMS{{\it J. London Math. Soc.}}
\def\JNT{{\it J. Number Theory}}
\def\PAMS{{\it Proc. Amer. Math. Soc.}}
\def\PLMS{{\it Proc. London Math. Soc.}}
\def\TAMS{{\it Trans. Amer. Math. Soc.}}


%Insertion de figures et illustrations
\def\picture #1 by #2 (#3){\leavevmode\vbox to #2{
     \hrule width #1 height 0pt depth 0pt
      \vfill
       \special{picture #3}}}

\def\illustration #1 by #2 (#3) scaled #4{\dimen1=#2
  \divide\dimen1 by 1000
  \multiply\dimen1 by #4
  \vtop to \dimen1{\dimen1=#1
  \divide\dimen1 by 1000
  \multiply\dimen1 by #4
  \hsize=\dimen1\vss
  \noindent\special{illustration #3 scaled #4}}}

%\input epsf.def
\def\figcentre#1#2{
$$\epsfysize=#2\epsfbox{#1}$$
}

\def\figure#1#2#3{
\vbox{\hskip #3mm\epsfysize=#2 mm\epsfbox{#1}}
}

\ifx\couleurs\oui
\def\illust#1#2{\includegraphics[height=#1]{#2}}
\fi


